To catch a chorus, verse, intro, or anything else: Analyzing a song with structural functions

Conventional music structure analysis algorithms aim to divide a song into segments and to group them with abstract labels (e.g., 'A', 'B', and 'C'). However, explicitly identifying the function of each segment (e.g., 'verse' or 'chorus') is rarely attempted, but has many applications. We introduce a multi-task deep learning framework to model these structural semantic labels directly from audio by estimating "verseness," "chorusness," and so forth, as a function of time. We propose a 7-class taxonomy (i.e., intro, verse, chorus, bridge, outro, instrumental, and silence) and provide rules to consolidate annotations from four disparate datasets. We also propose to use a spectral-temporal Transformer-based model, called SpecTNT, which can be trained with an additional connectionist temporal localization (CTL) loss. In cross-dataset evaluations using four public datasets, we demonstrate the effectiveness of the SpecTNT model and CTL loss, and obtain strong results overall: the proposed system outperforms state-of-the-art chorus-detection and boundary-detection methods at detecting choruses and boundaries, respectively.

==> Sec0_Misc.tex <==



% - more information = more useful for existing applications
%     - assisted navigation showing all function labels, not just choruses;
%     - more intelligent music retargeting (we can cite Adobe Audition)
%     - and ye, if you still think the current quality of thumbnails is sub-optimal, perhaps you can improve this with functional analysis.
% - enables new applications related to analysis of song fragments --- i.e., using MSA when full song not available.:
%     - improved understanding of song fragments.  (e.g., function-aware music tagging; you might estimate a song's tags differently if you think the input clip is a verse or chorus)
%     - synchronisation to other media (e.g., generating or retrieving video to match the audio)
%     - automatic mixing and mastering (e.g., what Landr does, but with effects tailored to the section type --- as suggested by \cite{nieto2020audio})
% - first step toward an ONLINE MSA method (currently would have a lag = half window size, but still! Not requiring context is a powerful leap to make.



% When listeners annotate the structure of a piece of music, they transcribe, with a set of boundary timestamps and segment labels, their holistic impression of how the piece is organized into sections of different types. If this sounds ambiguous and unrepeatable, that's because it is.

% In the field of Music Structure Analysis (MSA), most algorithms, including many recent and cutting-edge ones~\cite{mcfee2014analyzing, shibata2020music, wang2016structural}, use conventional features such as MFCCs and Pitch Class Profiles (PCPs).
% Devising a suitable feature for MSA is challenging, since so many aspects of music---including pitch, timbre, rhythm, and dynamics---impact the perception of structure~\cite{bruderer2009perception}.
% Some methods have aimed to combine input from multiple features~\cite{deberardinis2020unveiling}, but this requires care: MSA researchers have long been aware that structure at different timescales can be reflected best by different features (see, e.g.,~\cite{jehan2005a}).

% A common story in MIR in the past decade is that using feature learning can improve performance on a task. Although this wave of work arrived late to MSA, we have already seen the benefits of supervised learning to model, for instance, `what boundaries sound like'~\cite{ullrich2014_ismir}, or `what choruses sound like'~\cite{wang2021supervised}. One drawback of these two methods was that they were not compatible with existing MSA pipelines: new post-processing methods had to be conceived and implemented. Also, each one solved a limited version of MSA: segmentation and chorus detection, respectively. Developing a supervised approach that can explicitly minimize the losses of segmentation and labeling tasks at the same time remains a challenge.

% Directly identifying the structural functionalities is practically useful, because in many cases the input audio is not a full song but excerpt. Relying on self-similarity and clustering may fail when there is no obvious long-term repetition in the excerpt. 
% This is a key point to emphasise! Nothing else can achieve this yet. Maybe explain the application scenario more? The purpose?
% Important for auto/assisted editing tools: want to know the function of the sections in order to optimally rearrange them.


% In~\cite{mccallum2019unsupervised}, \textit{unsupervised} training was used to create a deep embedding of audio based on a triplet loss that aimed to reflect within-song similarity and contrast with a heuristic sampling technique. 
%The embedding vectors, treated as features, can directly replace traditional features in existing MSA pipelines, making it possible to leverage large, unannotated collections for MSA. 
% This approach demonstrates the promise of learning features with a deep neural network (DNN) for MSA.
%By introducing the triplet loss, it incorporates possible similar or dissimilar pairs of fragments within a song into a training objective.


% To sum up, we see motivation to design an MSA method that has three attributes: (1) uses learned features instead of traditional features; (2) uses supervised training, to take advantage of knowledge encoded by annotators; and (3) serves both segmentation and labeling tasks in MSA.

%An unsupervised approach has so far been sensible, given how few annotations exist, and how expensive it is to collect more. 


%                             %  APPEAL OF NEW DATA

% The appeal of supervised learning has grown with the introduction of Harmonix Set~\cite{nieto2019harmonix}, containing 912 annotated pop songs.
% Although Harmonix Set is smaller than SALAMI~\cite{smith2011design} (which has 1359 songs), it is much more consistent in terms of genre, which raises our hopes of learning a useful embedding.
% A model trained on SALAMI alone would have to adapt to the sound and structure of pop music, jazz standards, piano concertos, and more; a model trained on Harmonix Set has only to learn the sound and structure of pop songs.

%To the best of our knowledge, this work represents the first attempt to apply Transformer-based model to music structure analysis.



% SALAMI has a few examples from many musical domains; Harmonix has many examples from a relatively constrained domain.
% A model trained on SALAMI alone would have to adapt to the structure of pop music, jazz standards, piano concertos, and more, with only a few hundred examples per style; a model trained on Harmonix Set has only to learn the structure of pop songs, and has almost 1000 examples.
% With almost 1000 examples in a constrained domain (pop music), 
% In short, the time is right to pursue a supervised approach.
%912 examples for this--- almost quadruple the number of pop-music examples in SALAMI. 
% If a feature embedding is needed for another genre, the proposed approach would work as long as enough data were provided.
% \jordan{[Alternative closing sentence:] In the future, it would be interesting to compare genre-specific structure embeddings.}
% Also, a supervised approach permits inherent ability to well adapt to various genres when more relevant training data are available.


%Next section reviews related work. Section 3 describes our proposed training pipeline. In Section 4, we explain the choices we have made for each component, and in Section 5 we report experiments. 

%Since the learning objective will enforce the or, it 

% In this work, we aim to combine the value of supervision with the convenient interoperability of the metric learning approach to obtain an audio embedding useful for MSA.



% By introducing a modular pipeline including various training criterion and MSA algorithms, we make clear what parts of the system can be easily changed. 
% On three public datasets (HarmonixSet, SALAMI, and RWC), we demonstrate that using the learned features can improve an MSA algorithm significantly in intra- and inter-dataset evaluation scenarios.

% In the field of Music Structure Analysis (MSA), most algorithms, including some of the most recent and cutting-edge ones, rely on conventional features such as MFCCs and Pitch Class Profiles (PCPs).
% % In these algorithms, the hypothesis is that musical patterns will be expressed by these feat  ures.
% The choice of feature is crucial, since the goal of MSA algorithms is to search for patterns in audio---e.g., blocks and stripes in a self-similarity matrix (SSM) that exhibit   assume that the recurrence/block/stripe/regular structure they are looking for (whether recurrence,  a crucial role, since an
% % 
% However, machine learning approaches...
% % 
% Thanks to the advances of deep metric learning with more annotated data available, we are able to study the usefulness of the audio embeddings learned through a deep neural network in a supervised manner. In this paper, we propose a batch sampling scheme and a pipeline that 
% % In the history of music structure analysis (MSA) at ISMIR, there has been a greater focus on algorithm design---how to identify repetitions and changes, and how to deduce structure from these---than on feature design. 



% POINT 1.
% Previous methods for MSA have relied on careful feature selection.

% - At least since~\cite{jehan2005a}, MSA researchers have been aware that structure at different timescales can be reflected best by different features.
% - For example, spectral clustering~\cite{mcfee2014analyzing}, a SOTA music analysis algorithm, recommends using MFCCs to estimate local structure (since MFCCs are presumed to reflect timbre, which is presumed to be locally consistent), while chroma are used to estimate long-term structure (since chroma reflect pitch content, which is presumed to be the main evidence of large-scale repetitions).
% It is a reasonable hypothesis that features related to pitch and timbre content should be useful to modeling structure, but it should also be obvious that potentially many more factors---dynamics, tempo, performance variations, and who knows what else---also inform structure. Why is it obvious? Studies [smith2014, bruderer2013, ...] support the view that these other factors are important in the perception of musical structure; also, the observation that inter-annotator agreement for music structure is quite low [someone20XX] suggests that the perception of structure is either not a determinate process, or influenced by many individual factors---e.g., musical training and experience.

% There are 2 possibilities for why current methods fall short:
% 1 - our feature representation is incomplete and/or not tuned to a song/genre. (This can be the motivation why we think our model can help).
% 2 - our algorithm for identifying structure (based on novelty, homogeneity, repetition, etc. with respect to our feature representation) is incorrect or unreliable.
% In this work, we aim to learn a new feature representation to remove, as best as possible, any shortcoming in issue 1.
% We use this representation to improve existing methods---i.e., we do not attempt to resolve issue 2.
% % Stephen McAdams raised the question of what features in music are "form-bearing'': and the list is certainly longer than just timbre and pitch: dynamics, 




% POINT 2.
% Methods using learned representations have been proven as or more successful than methods using traditional features:
% - supervised training (to learn `what boundaries sound like', to learn 'what typical self-similarity lag matrices look like around boundaries) for segmentation by~\cite{ullrich2014_ismir, grill2015music}
% - unsupervised training (to learn `what makes two chunks sound similar') for obtaining a SSM (and thereafter apply traditional MSA, like Foote)~\cite{mccallum2019unsupervised}
% - supervised training (to learn how MFCCs, CQT, other traditional features, generate structures) to predict segmentation AND labeling by~\cite{shibata2020music}
% - supervised training (to learn what `chorusness' sounds like) by ~\cite{wang2021supervised}

% In general terms, the pipeline of an MSA algorithm progresses from point A (audio) to point B (feature representation) to each part of the estimated structure: points C (boundaries), D (abstract labels that express grouping, like ``A'', ``B'', etc.), and E (semantic labels that express meaning, like ``chorus'' or ``intro'').

% Training has been used to improve many of these connections:

%~\cite{ullrich2014_ismir, grill2015music} used supervised training to learn what characterises boundaries in audio: this established a direct path from A to C.

%~\cite{shibata2020music} used supervision to model how traditional features (MFCCs, CQT, etc.) relate to music structure; i.e., a model for going from B->(C,D) jointly.

%~\cite{wang2021supervised} used supervision to learn how what characterises both boundaries and ``chorusness'' in audio, hence making a direct link from A->(C,E)---however, since only two labels are considered (chorus and non-chorus), the predicted structures were not the typical kind. Also, the authors speculated that this method may not be extendable to other segment labels since most labels (after chorus, verse, intro and outro) are more rare and ambiguous.

%~\cite{mccallum2019unsupervised} used unsupervised training to learn a general music similarity metric suitable for MSA, aiming to improve the path from A to B. They showed that with this metric they could improve performance on estimating C. The same feature would have been usable to estimate D using typical approaches but was not tested. The model aimed to learn a general notion of similarity: what makes two chunks of audio sound similar? They used a rough but clever heuristic---proximity in time within a song---as a guess for whether two clips should sound similar.



% what makes two  makes two chunks sound similar') for obtaining a SSM (and thereafter apply traditional MSA, like Foote) 


%  We might also use traditional features, but then use supervision to establish how to predict the  supervision to 


% When an MIR task faces a performance ceiling, a common strategy is to apply deep learning to devise a better feature representation.
% This has been done for MSA in a few cases, including:
% supervised training to learn what characterises boundaries between sections~\cite{ullrich2014_ismir, grill2015music};
% unsupervised training to learn what makes 


% first,~\cite{ullrich2014_ismir} used supervised training to learn a model of what spectra centered on a boundary look like; the approach was revised in~\cite{grill2015music} to learn a model of what areas of a self-similarity lag matrix look like. Both approaches set new standards for the state of the art in boundary detection.





% POINT 3. (Summing up shortcomings from previous work)
% None of these methods satisfies this full set of attributes:
% - learned features instead of traditional features (learning promises improvement)
% - supervised training (we want to take advantage of segment labels provided by existing annotations of structure)
% - tested on \textbf{both} tasks involved in MSA: segmentation and labeling

% POINT 4.
% We propose a method that DOES do all of this.
% [Expand on this briefly, but in a bit more detail, highlighting the main novelties and the other achievements of our paper.]
% - Propose and compare several sampling strategies
% - We explain this system as a modular pipeline, making clear what parts of the system are easily changed.
% - We evaluate our system on three datasets (SALAMI, Harmonix and RWC) to measure the success of our system at intra- and inter-dataset modeling of similarity.
% etc
% etc

% Another issue with prior work: the training corpus (SALAMI) is large (over 1000 tracks), but perhaps too diverse: a model trained on SALAMI is attempting to explain the structure of pop music, prog rock, jazz standards, piano concertos, choral works, and more. However, most of the intuition behind structure analysis methods is guided by theory applicable to pop music but perhaps not these other types of songs. In this work, we use a subset of SALAMI categorised as 'pop', along with the recent Harmonix Set which contains only pop.

% \section{Related work}

% Many MSA approaches (see~\cite{nieto2020audio} for an overview) are supervised in the sense of being tuned to a dataset---e.g., by setting a filter size according to the average segment duration in a corpus. 
% % Speaking broadly, we might view any method that has been tuned to a dataset---e.g., by setting a filter size according to the average segment duration in a corpus---as being supervised.
% An advanced version of this is~\cite{mcfee2014learning}, in which a recurrence matrix is transformed to match the statistics of a training dataset.
% However, supervised training has only been used in a few instances for MSA.

% % Defining supervision more narrowly, supervised training has been used in only a few instances for MSA.
% The first such method used supervision to learn a notion of `boundaryness' directly from audio~\cite{ullrich2014_ismir}; the method was refined to use a self-similarity lag matrix computed from audio~\cite{grill2015music}.
% % The first such method was~\cite{ullrich2014_ismir}, who used supervision to learn a notion of `boundaryness' directly from audio; the method was refined in ~\cite{grill2015music} to use a self-similarity lag matrix computed from audio.
% Similarly,~\cite{wang2021supervised} used supervision to learn what characterizes boundaries as well as ``chorusness'' in audio, and used it in a system to predict the locations of choruses in songs, which is a subproblem of MSA.
% Although these 3 systems all have an `end-to-end' flavor, in fact they required the invention of new custom pipelines to obtain estimates of structure, e.g., a peak-picking method to select the likeliest set of boundaries from a boundary probability curve.
% % A hybrid system combined with a CNN-based boundary model, a timbre homogeneity model, and a segment duration model~\cite{maezawa2019music}.
% The post-processing is also complex in~\cite{maezawa2019music}, in which a boundary fitness estimator similar to~\cite{grill2015music} is combined in a hybrid model with a trained segment length fitness estimator and a hand-crafted timbral homogeneity estimator.
% % In order to discover a segmentation that maximises all of these fitnesses, a novel beam-search approach was proposed.
% In our work, we aim to arrive at a feature representation that can be used with existing pipelines.

% % The segmentation that maximizes all of these fitness functions is sought using beam search.
% Taking the converse approach,~\cite{shibata2020music} used supervision to model how traditional features (MFCCs, CQT, etc.) relate to music structure, using an LSTM combined with a Hidden semi-Markov Model. Since our approaches are complementary, a combined approach---inputting deep structure features to the LSTM-HSMM---may prove successful, and should be explored in future work.
% combining them should be explored in future work a combination of the approaches work targets an independent part of the In this work, we take the complementary approach: using supervision to learn the features that can be employed directly by existing MSA methods. A combination of both methods is a potential avenue for future work.

% But maybe we can skip this?

%We train a feature representation that can be directly plugged into existing MSA pipelines.

%- Unsupervised feature learning for boundary detection:~\cite{mccallum2019unsupervised} uses unsupervised training to learn a general music similarity metric suitable for MSA. Our work resembles this one closely, but with several differences.
%- batch processing method differs?
%- ours is supervised, of course!
%- they only tested their feature in a segmentation task, although it could have been used directly to estimate segment labeling too. We do both tasks: segmentation and labeling.

%Training a deep neural network model with a metric learning technique to generate music structure features has been studied in~\cite{mccallum2019unsupervised}. However, this prior work does not explore the section annotations as supervision, instead it exploits the time proximity of audio features, assuming that audio fragments nearby one another on the time axis belong to the same section. This may limit the model generalizability since the assumption does not hold when the fragments are around the section boundary. Two fragments respectively from two repeated sections far apart can be similar. 

% As noted in the previous section, metric learning was previously applied to improve MSA by~\cite{mccallum2019unsupervised}, but that work took an unsupervised approach: audio fragments in a piece were presumed to belong to the same class if they were near each other in time, and to different classes otherwise. This is a useful heuristic, but by design we expect it to use many false positive and false negative pairs in training.
% Of course, given the multidimensional nature of music similarity, the heuristic has clear limitations.
% Regarding unsupervised feature learning, the idea of~\cite{mccallum2019unsupervised} resembles ours closely, but with several key differences. It trained a DNN using heuristics to compose the time proximity for training pairs without supervisions from the annotations.
% Also, that work did not report any evaluation on whether the learned embeddings could help with the segment labeling task, nor on the impact of many choices made in the system that could affect the results: the model architecture, loss function, and segmentation method.
% In this work, we conduct evaluations on the segmentation and labeling tasks, and investigate the impact of these design choices.
% In terms of ablation study, the choice of model architecture, loss function, and segmentation method is monotonic. It is not clear whether choosing a different module can impact the output result significantly.
% The supervision strategy in this work differs from prior art, and to our knowledge, this work represents the first attempt to develop supervised feature learning with a goal of improving existing MSA algorithms. 

% A representative sample of traditional MSA approaches are implemented in MSAF~\cite{nieto2016systematic}; in this work, we use
% spectral clustering~\cite{mcfee2014analyzing}, Convex-NMF~\cite{nieto2013convex}, and FMC2D~\cite{nieto2014music}.
% We note that each is based on analyzing some version of a self-similarity matrix. Please refer to the papers for details. 
% An overview of MSA algorithms, corpora and evaluation methods is provided by~\cite{nieto2020audio}.



% The review paper nieto
% 1. Traditional boundary detection focused:
% Time series structure features~\cite{serra2012unsupervised}.
% Novelty curve and checkerboard kernel~\cite{foote2000automatic}.
%
% 2. Unsupervised feature learning for boundary detection:
% unsupervised learning of deep features for music segmentation~\cite{mccallum2019unsupervised}.
% 
% 
% 3. Supervised boundary detection:
% A convolutional neural network (CNN)to detect whether the center of a 16-second input is a boundary~\cite{ullrich2014_ismir,grill2015music}.
% Using ordinal linear discriminant analysis (OLDA) technique to learn feature transformation~\cite{mcfee2014learning}.
% 
% 4. Supervised MSA:
% paired a standard structure analysis system with an HMM trained to label the sections~\cite{paulus2009music}.
% a hierarchical generative model (with section parts generating chord progressions, and these in turn generating observed feature sequences)~\cite{shibata2020music}.
% 
% 
% 
%[optional] deep metric learning in MIR tasks. There are several in auto-tagging. [see Juhan Nam's publication~\cite{nam2018deep}]

%\begin{figure}
%\centering  
%\subfigure[Figure A]{\label{fig:tcn}\includegraphics[width=0.30\columnwidth]{figs/tcn.pdf}}
%\subfigure[Figure B]{\label{fig:specTNT}\includegraphics[width=0.30\columnwidth]{figs/specTNT.pdf}}
%\subfigure[Figure B]{\label{fig:specTNT_tcn}\includegraphics[width=0.30\columnwidth]{figs/specTNT_tcn.pdf}}
%\caption{Overview of the proposed model structures, TCN, SpecTNT and SpecTNT-TCN.}
%\end{figure}


